Centralised Multimode Power Oscillation Damping Controller for Photovoltaic Plants with Communication Delay Compensation

Low-frequency oscillations are an inherent phenomena in transmission networks and renewable energy plants should be configured to damp them. Commonly, a centralised controller is used in PV plants to coordinate PV generators via communication channels. However, the communication systems of PV plants introduce delays of a stochastic nature that degrade the performance of centralised control algorithms. Therefore, controllers for oscillation damping may not operate correctly unless the communication channel characteristics are not considered and compensated. In this paper, a centralised controller is proposed for the oscillation damping that uses a PV plant with all the realistic effects of communication channels taken into consideration. The communication channels are modelled based on measurements taken in a laboratory environment. The controller is designed to damp several modes of oscillation by using the open-loop phase shift compensation. Theoretical developments were validated in a laboratory using four converters acting as two PV inverters, a battery and a STATCOM. A real-time processing platform was used to implement the centralised controller and to deploy the communication infrastructure. Experimental results show the communication channels impose severe restrictions on the performance of centralised POD controllers, highlighting the importance of their accurate modelling and consideration during the controller design stage.

==> FIGURES/Style.tex <==
\usepackage{tikz}
\usetikzlibrary{positioning,shapes,arrows.meta,patterns,calc}
\usepackage[european,american inductors,siunitx]{circuitikz}
\usepackage{pgfplots}
\usepgfplotslibrary{groupplots}
\pgfdeclarelayer{points}
\pgfsetlayers{main,points}
% \pgfplotsset{compat=1.12,}
\pgfplotsset{compat=1.15}
 %            ylabsh/.style={every axis y label/.style={at={(0,0.7)}, xshift=#1, rotate=90}}}

% Text colors
\definecolor{Tred}{rgb}{0.68, 0.05, 0.0}
\definecolor{Tgreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{Torange}{rgb}{0.95, 0.52, 0.04}
\definecolor{Tyellow}{rgb}{1.0, 0.73, 0.0}
\definecolor{Tblue}{rgb}{0.28, 0.57, 0.81}

% Matlab default - new version from R2014b
\definecolor{blue_m}{rgb}{0, 0.4470, 0.7410}
\definecolor{orange_m}{rgb}{0.8500, 0.3250, 0.0980}
\definecolor{yellow_m}{rgb}{0.9290, 0.6940, 0.1250}
\definecolor{purple_m}{rgb}{0.4940, 0.1840, 0.5560}
\definecolor{green_m}{rgb}{0.4660, 0.6740, 0.1880}
\definecolor{lightblue_m}{rgb}{0.3010, 0.7450, 0.9330}
\definecolor{blue_m}{rgb}{0, 0.4470, 0.7410}
\definecolor{red_m}{rgb}{0.6350, 0.0780, 0.1840}
\definecolor{gray_m}{rgb}{0.529, 0.529, 0.529}
\definecolor{gray_m_fill}{rgb}{0.952, 0.952, 0.952}


% BuRD diverging color scheme
% Source: https://personal.sron.nl/~pault/
\definecolor{red4}{rgb}{0.698, 0.094, 0.169}
\definecolor{red3}{rgb}{0.839, 0.376, 0.302}
\definecolor{red2}{rgb}{0.957, 0.647, 0.51}
\definecolor{red1}{rgb}{0.992, 0.859, 0.78}
\definecolor{white}{rgb}{0.969, 0.969, 0.969}
\definecolor{blue1}{rgb}{0.820, 0.890, 0.940}
\definecolor{blue2}{rgb}{0.573, 0.773, 0.871}
\definecolor{blue3}{rgb}{0.263, 0.576, 0.765}
\definecolor{blue4}{rgb}{0.129, 0.4, 0.675}

% Figure 3: Vibrant qualitative colour scheme
% Source: https://personal.sron.nl/~pault/
\definecolor{orange_q}{rgb}{0.933, 0.466, 0.2}
\definecolor{blue_q}{rgb}{0, 0.466, 0.733}
\definecolor{cyan_q}{rgb}{0.2, 0.733, 0.933}
\definecolor{magenta_q}{rgb}{0.933, 0.2, 0.466}
\definecolor{red_q}{rgb}{0.8, 0.2, 0.066}
\definecolor{teal_q}{rgb}{0, 0.6, 0.533}
\definecolor{gray_q}{rgb}{0.733, 0.733, 0.733}
\tikzset{
    bus/.style =  {
                    draw,
                    line width=0.3mm,
                    line cap=round},
    load/.style = {
                    draw,
                    thick,
                    regular polygon,
                    regular polygon sides=3,
                    shape border rotate=180,
                    minimum width=1mm,
                    inner sep=1.5pt,
                    fill=white},
    grid_line/.style = {
                        draw,
                        line cap=round},
    PE_block/.style =  {
                        draw,
                        rectangle,
                        anchor=east,
                        minimum height = 1cm,
                        minimum width = 1cm},
    block/.style =  {
                    draw,
                    rectangle,
                    minimum height = 2em,
                    minimum width = 2em,
                    inner sep=0.4mm,
                    outer sep=0mm,},
    sum_PN_1/.style =   {
                        draw,
                        circle,
                        minimum width = 0.4cm},
    saturation/.style={
                        draw,
                        minimum height = 2em,
                        minimum width = 2em,
                        path picture={
                                        \pgfpointdiff{
                                            \pgfpointanchor{path picture bounding box}{north east}}
                                        {\pgfpointanchor{path picture bounding box}{south west}}
                                        \pgfgetlastxy\x\y
                                        % Scale the x and y vectors so that the range
                                        % -1 to 1 is slightly shorter than the size of the node
                                        \tikzset{x=\x*.4, y=\y*.4};
                                        % Draw annotation
                                        \draw [ultra thin] (-1,0) -- (1,0) (0,-1) -- (0,1); 
                                        \draw (-1,-.7) -- (-.4,-.7) -- (.4,.7) --      (1,.7);}},
    droop/.style={
                        draw,
                        minimum height = 2em,
                        minimum width = 2em,
                        path picture={
                                        \pgfpointdiff{
                                            \pgfpointanchor{path picture bounding box}{north east}}
                                        {\pgfpointanchor{path picture bounding box}{south west}}
                                        \pgfgetlastxy\x\y
                                        % Scale the x and y vectors so that the range
                                        % -1 to 1 is slightly shorter than the size of the node
                                        \tikzset{x=\x*.4, y=\y*.4};
                                        % Draw annotation
                                        \draw [ultra thin] (0.7,0.7) -- (-0.7,0.7) (0.7,0.7) -- (0.7,-0.7);
                                        \draw (0.958,-0.4) -- (-0.7,0);
                                        }},
    gain/.style =  {
                    draw,
                    isosceles triangle,
                    isosceles triangle stretches,
                    anchor=left corner,
                    inner sep=0.5mm,
                    outer sep=0mm,},
    quest/.style = {
                    diamond,
                    draw,
                    minimum height = 1cm,
                    minimum width = 1cm,
                    text centered, 
                    aspect=2},  
    -|-/.style={
                to path={
                        (\tikztostart) -|($(\tikztostart)!#1!(\tikztotarget)$) |-(\tikztotarget)
                        \tikztonodes}},
    -|-/.default=0.5,
    set point size/.code={\pgfmathsetmacro{\pointsize}{sqrt(\pgflinewidth)}},
    point size/.style={set point size/.prefix style={line width=#1}},
    every dot/.style = {inner sep=0, outer sep=0,font=},
    outer dot/.style = {every dot, scale=4*\pointsize},
    inner dot/.style = {every dot, scale=\pointsize, text=#1}, inner dot/.default={black},
    point fill/.style = {inner dot/.default={#1}},
    point coordinate/.style={insert path={coordinate(#1)}},
    point/.style={insert path={
      node[inner sep=0, overlay, every point/.try, #1, set point size,
        path picture={
          \begin{pgfonlayer}{points}
            \node[outer dot]{.} node[inner dot]{.};
          \end{pgfonlayer}
        }
      ]
    }
  }
}
